Mirror Manifolds in Higher Dimension

We describe mirror manifolds in dimensions different from the familiar case of complex threefolds. We emphasize the simplifying features of dimension three and supply more robust methods that do not rely on such special characteristics and hence naturally generalize to other dimensions. The moduli spaces for Calabi--Yau $d$-folds are somewhat different from the ``special K\"ahler manifolds'' which had occurred for $d=3$, and we indicate the new geometrical structures which arise. We formulate and apply procedures which allow for the construction of mirror maps and the calculation of order-by-order instanton corrections to Yukawa couplings. Mathematically, these corrections are expected to correspond to calculating Chern classes of various parameter spaces (Hilbert schemes) for rational curves on Calabi--Yau manifolds. Our results agree with those obtained by more traditional mathematical methods in the limited number of cases for which the latter analysis can be carried out. Finally, we make explicit some striking relations between instanton corrections for various Yukawa couplings, derived from the associativity of the operator product algebra.

==> tables.tex <==
%
% This file produces the tables for ``Mirror manifolds in higher dimension'',
% by B. R. Greene, D. R. Morrison, and M. R. Plesser.
%
% It uses harvmac to find your local ``landscape'' command.  
%
% The file must be TeX-ed using harvmac's ``big'' (portrait) mode, but
% printing must be done in landscape (harvmac's ``little'') mode.
%
% We have also included a PostScript file (optimized for 300dpi) which 
% could be printed directly as an alternative.
%

\input harvmac.tex

\ifx\answ\bigans
\else\immediate\write16{ THESE TABLES MUST BE PROCESSED IN `BIG' MODE.} 
\end \fi

\redoffs
\vsize=7truein
\hsize=10truein

\output={
\shipout\vbox{\speclscape\makeheadline\pagebody}\advancepageno}

\font\eightrm=cmr8 \font\eighti=cmmi8
\font\eightsy=cmsy8 \font\eightbf=cmbx8
\font\eightit=cmti8 \font\eightsl=cmsl8 \skewchar\eighti='177
\skewchar\eightsy='60

\def\eightpoint{\def\rm{\fam0\eightrm}% switch to eightpoint font
\textfont0=\eightrm \scriptfont0=\fiverm \scriptscriptfont0=\fiverm
\textfont1=\eighti \scriptfont1=\fivei \scriptscriptfont1=\fivei
\textfont2=\eightsy \scriptfont2=\fivesy \scriptscriptfont2=\fivesy
\textfont\itfam=\eighti
\def\it{\fam\itfam\eightit}\def\sl{\fam\slfam\eightsl}%
\textfont\bffam=\eightbf \def\bf{\fam\bffam\eightbf}\rm}

%\hfuzz=100cm

{\eightpoint
\def\tablerule{\noalign{\hrule}}
\def\ilspace{\omit&height1pt&&&&\cr}
$$\vbox{\tabskip=0pt \offinterlineskip
\halign{\strut#&
\vrule#&\hfil\quad$#$\quad\hfil&\vrule#&\quad$#$\quad\hfil&
\vrule#\cr \tablerule\ilspace
&&d&&\hbox{$d$-point functions}&\cr\ilspace\tablerule\ilspace
&&4&&
6 + 120960 \,q + 4136832000 \,q^2  + 148146924602880 \,q^3  +
    5420219848911544320 \,q^4  + 200623934537137119778560 \,q^5  +
    7478994517395643259712737280 \,q^6  
&\cr\ilspace
&&&& \quad {} +
 280135301818357004749298146851840 \,q^7  + 
    10528167289356385699173014219946393600 \,q^8  + 
    396658819202496234945300681212382224722560 \,q^9  
&\cr\ilspace
&&&& \quad {} + 
    14972930462574202465673643937107499992165427200 \,q^{10}   + 
    566037069767251121484562070892662863943365345190400 \,q^{11}   + 
%    21424151141341932048068067497996096856724987411324108800 \,q^{12} +
 \dots
&\cr\ilspace\tablerule\ilspace
&&5&&
7 + 3727381 \,q + 2637885990187 \,q^2  + 1927092954108108787 \,q^3  +
1425153551321014327663291 \,q^4  + 1060347883438857662557634869906 \,q^5
&\cr\ilspace
&&&& \quad {} +
    791661306374088776109692880989252173 \,q^6  + 
    592348256908461616176898022359492565546566 \,q^7  
&\cr\ilspace
&&&& \quad {} + 
    443865568545713063761643598030194801299861575595 \,q^8  + 
    332947403131697202086626568381790256001850741509664373 \,q^9  + 
%    249936692470870793855154463327623520938049650517355107703502 \,q^{10} +
\dots
&\cr\ilspace\tablerule\ilspace
&&6&&
8 + 106975232 \,q + 1672023727001600 \,q^2  + 26611692333081695092736 \,q^3  +
    426129121674687823674948571136 \,q^4  
&\cr\ilspace
&&&& \quad {} +
    6842148599241293047857339542861643776 \,q^5  +
    110018992594692024449889564415904439556898816 \,q^6   
&\cr\ilspace
&&&& \quad {} +
    1770551943055574073245974844490813198478975912902656 \,q^7  +
    28508925683951911989843155602330000507452539542539447947264 \,q^8  + 
%    459205926175034196299831853449290667032138952707194903528763228160 \,q^9  + 
%   7398469444880346316901605849057839986326194349089322436910222882551234560
%   \,q^{10} +
 \dots
&\cr\ilspace\tablerule\ilspace
&&7&&
9 + 3103936929 \,q + 1165013014173543657 \,q^2  +
    441297815019235844688286425 \,q^3  +
    167606183678231435989321323352019097 \,q^4  
&\cr\ilspace
&&&& \quad {} +
    63725266235392545772891574625466284314384997 \,q^5  + 
    24241288949516830588590880856230885330230589276883697 \,q^6   
&\cr\ilspace
&&&& \quad {} +
    9224015119655326077755094748604809293729079769166286338124125 \,q^7  + 
%    3510387442646708119296403605538516380798634576250170024146401252896857 
%     \,q^8  
 \dots
&\cr\ilspace\tablerule\ilspace
&&8&&
10 + 94327552000 \,q + 930496455109619200000 \,q^2  +
    9217712440694086335170560000000 \,q^3  + 
    91408512461766539388538224090616000000000 \,q^4   
&\cr\ilspace
&&&& \quad {} +
    906798958458710503048638459436511928645436567552000 \,q^5  + 
    8997152189131293850735805864983772379107049616519528407040000 \,q^6   
&\cr\ilspace
&&&& \quad {} +
    89275777693040346906449878258202162124048469440553887673238192128000000 
     \,q^7 +
 \dots
&\cr\ilspace\tablerule\ilspace
&&9&&
11 + 3049747360561 \,q + 865196274264724937872931 \,q^2  +
    245891784376657937170481797615461001 \,q^3  
&\cr\ilspace
&&&& \quad {} +
    69909581514948393506313481730554975387628730971 \,q^4  + 
    19878335509713026535802529940943471736182876279710737890681 \,q^5   
&\cr\ilspace
&&&& \quad {} +
    5652532179569595758241560307343719407665962471280448209489098916126883 
     \,q^6  + 
 \dots
&\cr\ilspace\tablerule\ilspace
&&10&&
12 + 105530993897472 \,q + 938751865652732974917414912 \,q^2  +
    8356637011952074628498424363753120202752 \,q^3  
&\cr\ilspace
&&&& \quad {} +
    74398936834441392566214936916906628540271882474811392 \,q^4  + 
    662394452847740708498379623076592060042553944377293453096800223232 \,q^5  
&\cr\ilspace
&&&& \quad {} +
   589755241941434343638761082760255175714657880143896940423903673544310628%
0767488 \,q^6  + 
 \dots
%&\cr\ilspace\tablerule\ilspace
&\cr
\tablerule
\noalign{\vskip2pt}
&\multispan{5}\hfil \tenpoint
Table 1: $d$-point functions in dimension $d$\hfil\cr
}}$$
}

\vfill\eject

\def\frac#1#2{{{#1}\over{#2}}}
\def\cue#1{\frac{q^{#1}}{1-q^{#1}}}
\def\q{\cue{}}
\def\qq{\cue2}
\def\qqq{\cue3}
\def\qqqq{\cue4}
\def\qqqqq{\cue5}
\def\qqqqqq{\cue6}

%\strut#&
%\vrule#&\hfil\quad$#$\quad\hfil&\vrule#&\hfil\quad$#$\quad\hfil&
%\vrule#\cr

{\eightpoint
\def\tablerule{\noalign{\hrule}}
\def\ilspace{\omit&height1pt&&&&\cr}
$$\vbox{\tabskip=0pt \offinterlineskip
\halign{\strut#&
\vrule#&\hfil\quad$#$\quad\hfil&\vrule#&\quad$#$\quad\hfil&
\vrule#\cr \tablerule\ilspace
&&d&&\hbox{Three-point functions}&\cr\ilspace\tablerule\ilspace
&&4&&
Y_1^1=6+60480\q+1763536320\qq+56296406496960\qqq
+1883452671845660160\qqqq+64779403909220549640000\qqqqq\dots
&\cr\ilspace\tablerule\ilspace
&&5&&
Y_1^1=7+1009792\q+488959144352\qq+274758045709320936\qqq
+166051192150334178451456\qqqq
%+104782774271335261727812676000\qqqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&5&&
Y_2^1=7+1707797\q+1021575491286\qq+667645611326779470\qqq
+454542525929947966588896\qqqq
%+316703622311920552513195121325\qqqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&6&&
Y_1^1=8+15984640\q+133588638826496\qq+1386812286427872761856\qqq
+16010798260253954110394728448\qqqq+\dots
&\cr\ilspace\tablerule\ilspace
&&6&&
Y_2^1=8+37502976\q+448681408315392\qq+6002251230562024144896\qqq
+84488476029298653829523177472\qqqq+\dots
&\cr\ilspace\tablerule\ilspace
&&6&&
Y_2^2=8+59021312\q+821654025830400\qq+12197109744970010814464\qqq
+186083410628492378226388631552\qqqq+\dots
&\cr\ilspace\tablerule\ilspace
&&7&&
Y_1^1=9+253490796\q+39031273362637440\qq
+8078045888048061054330324\qqq
+1935263133090844196814494099500032\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&7&&
Y_2^1=9+763954092\q+187554590257349088\qq
+53621695689211084188650940\qqq
+16467077347090342394985001860453504\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&7&&
Y_3^1=9+1069047153\q+312074852318965368\qq
+101447807418804760300649304\qqq
+34554976338508396442154650827251216\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&7&&
Y_2^2=9+1579510449\q+506855012110118424\qq
+174633921378662035929052320\qqq
+62036347648424671947435351078921912\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&8&&
Y_1^1=10+4120776000\q+12607965435718224000\qq
+56689974104916623862439224000\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&8&&
Y_2^1=10+15274952000\q+80684596772238448000\qq
+524473167338866432254165048000\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&8&&
Y_3^1=10+27768048000\q+200581960800610752000\qq
+1639883435802047356497671952000\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&8&&
Y_2^2=10+38922224000\q+295035175517918176000\qq
+2467449594491156931046837776000\qqq
%+21585952449297725966376014809800409600000\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&8&&
Y_3^2=10+51415320000\q+444475303469701680000\qq
+4089048226644406809222184680000\qqq
%+38593212249861107841832963566199008000000\qqqq
+\dots
%&\cr\ilspace\tablerule\ilspace
&\cr
\tablerule
\noalign{\vskip2pt}
&\multispan{5}\hfil \tenpoint
Table 2: Three-point functions in dimension $d$, $4\le d\le8$\hfil\cr
}}$$
}

\vfill\eject

{\eightpoint
\def\tablerule{\noalign{\hrule}}
\def\ilspace{\omit&height1pt&&&&\cr}
$$\vbox{\tabskip=0pt \offinterlineskip
\halign{\strut#&
\vrule#&\hfil\quad$#$\quad\hfil&\vrule#&\quad$#$\quad\hfil&
\vrule#\cr \tablerule\ilspace
&&d&&\hbox{Three-point functions}&\cr\ilspace\tablerule\ilspace
&&9&&
Y_1^1=11+69407571816\q+4565325719860021608624\qq
+486831084305817727642305709925784\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&9&&
Y_2^1=11+307393401172\q+37005001823802188657624\qq
+5868069805933786797109659387704124\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&9&&
Y_3^1=11+695221679878\q+127922335050535174614916\qq
+27500598436953801920237040452936322\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&9&&
Y_4^1=11+905702054829\q+193693669320390878077186\qq
+46631251296278131748940806631976872\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&9&&
Y_2^2=11+933207509234\q+173901546566279203106468\qq
+37310808146135703367927046095148086\qqq
%+8568373602025384931095443488446969678498023104\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&9&&
Y_3^2=11+1531516162891\q+364629304647788940660824\qq
+93483169112936030274354586771249766\qqq
%+24736745753321562724483530726693623147881119002\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&9&&
Y_3^3=11+1919344441597\q+498705676383823268404990\qq
+135578347091808508663450919122287332\qqq
%+37503368022986711789110169990347402780071063004\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&10&&
Y_1^1=12+1217507106816\q+1861791822397620935737344\qq
+5128660247833325056966281364761206784\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&10&&
Y_2^1=12+6306655500288\q+18415607624138339954786304\qq
+76684904282498644296301812327894878208\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&10&&
Y_3^1=12+17225362851840\q+83885220561474498867757056\qq
+499293309557937087326375598615454660608\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&10&&
Y_4^1=12+28015971489792\q+179982840924749584358866944\qq
+1316838352593364835173763931348327770112\qqq+\dots
&\cr\ilspace\tablerule\ilspace
&&10&&
Y_2^2=12+22314511245312\q+107227899142191919158312960\qq
+627029137534107622315490005905787576320\qqq
%+4043964444297867321863061713130539496069864925298688\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&10&&
Y_3^2=12+44023827234816\q+297755098999730079369412608\qq
+2228162463490181234075299799539491962880\qqq
%+17459305242953752701942423872031637493025939973079040\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&10&&
Y_4^2=12+54814435872768\q+417950364467570984815214592\qq
+3418037850981202953204910537008894799872\qqq
%+28765635488346936207012805840908858273150037838659584\qqqq
+\dots
&\cr\ilspace\tablerule\ilspace
&&10&&
Y_3^3=12+65733143224320\q+527556832251612742800359424\qq
+4445632319073239456054488536360314019840\qqq
%+38195900907247151509784916874176490949252016517545984\qqqq
+\dots
&\cr
\tablerule
\noalign{\vskip2pt}
&\multispan{5}\hfil \tenpoint
Table 3: Three-point functions in dimension $d$, $d=9,10$\hfil\cr
}}$$
}

\bye


